An Empirical Study on Budget-Aware Online Kernel Algorithms for Streams of Graphs

Kernel methods are considered an effective technique for on-line learning. Many approaches have been developed for compactly representing the dual solution of a kernel method when the problem imposes memory constraints. However, in literature no work is specifically tailored to streams of graphs. Motivated by the fact that the size of the feature space representation of many state-of-the-art graph kernels is relatively small and thus it is explicitly computable, we study whether executing kernel algorithms in the feature space can be more effective than the classical dual approach. We study three different algorithms and various strategies for managing the budget. Efficiency and efficacy of the proposed approaches are experimentally assessed on relatively large graph streams exhibiting concept drift. It turns out that, when strict memory budget constraints have to be enforced, working in feature space, given the current state of the art on graph kernels, is more than a viable alternative to dual approaches, both in terms of speed and classification performance.

==> fscore_ince.tex <==


\subsection{Feature Selection for Budget Management} \label{sec:fs}

Since any kernel method using the kernel functions in \cite{Shervashidze2009a, Costa2010, Dasan2012} can be performed in the primal space, it is possible to apply {\it feature selection} techniques, i.e. deleting non-informative features, in order to reduce noise in the data and the size of the model \cite{Chen}. 
A typical approach is to compute a statistical measure for estimating the relevance of each feature w.r.t. the target concept, and 
 to discard the less-correlated features. An example of such measure is the F-score \cite{Chen}. 
In the traditional batch scenario, the F-score of a feature $i$ is defined for binary  classification tasks as follows:
\begin{equation} 
F\!s(i) = \displaystyle \cfrac{(AVG_{i}^{+} - AVG_i)^2 + (AVG_{i}^{-} - AVG_i)^2} { \cfrac{\displaystyle\sum_{j \in Tr^{+}} (f^{j}_{i} - AVG_{i}^{+})^2}{ |Tr^{+}| - 1} + \cfrac{ \displaystyle\sum_{j \in Tr^{-}} (f^{j}_{i} - AVG^{-}_{i})^2} {|Tr^{-}| -1}     }
\label{eq:fscore}
\end{equation}
\noindent where $AVG_{i}$ is the average frequency of feature $i$ in the dataset, $AVG_{i}^{+}$ ($AVG_{i}^{-}$) is the average frequency of feature $i$ in positive (negative) examples, $|Tr^{+}|$ ($|Tr^{-}|$) is the number of positive (negative) examples and $f^{j}_{i}$ is the frequency of feature $i$ in the $j^{th}$ example of the dataset. Features that get small values of F-score are not very informative with respect to the binary classification task. 
Eq.~(\ref{eq:fscore}) cannot be applied as is to a stream since instances arrive one at time. As a minor contribution, we rewrite an incremental version of the F-score. 
Let ${\cal I}^+_t$  (${\cal I}^-_t$) be the set of positive (negative) instances which have been observed from the stream after having read $t$ instances, then the F-score $F\!s(i,t)$ can be rewritten by using the following quantities:
\[ n^+_t = | {\cal I}^+_t|,\ \ \ f^{+}_i(t) = \sum_{j\in {\cal I}^+_t} f^{j}_{i},\ \ \  f^{2,+}_i(t) = \sum_{j\in {\cal I}^+_t} (f^{j}_{i})^2\]
\[n^-_t = |{\cal I}^-_t|, \ \ \ f^{-}_i(t) = \sum_{j\in {\cal I}^-_t} f^{j}_{i}, \ \ \ f^{2,-}_i(t) = \sum_{j\in {\cal I}^-_t} (f^{j}_{i})^2.\]
In fact, we have:
\[AVG_{i,t}^{+} = \frac{f^{+}_i(t)}{n^+_t}, \ AVG_{i,t}^{-} = \frac{f^{-}_i(t)}{n^-_t}\]
\[ AVG_{i,t} = \frac{f^{+}_i(t)+f^{-}_i(t)}{n^+_t + n^-_t} \]
and
\begin{equation} 
F\!s(i,t) = \displaystyle \cfrac{(AVG_{i,t}^{+} - AVG_{i,t})^2 + (AVG_{i,t}^{-} - AVG_{i,t})^2} { D^+_t + D^-_t     }
\label{eq:fscore-inc}
\end{equation}
where 
\[D^+_t = \frac{f^{2,+}_i(t) -2AVG_{i,t}^{+}f^{+}_i(t)  +n^{+}_t (AVG_{i,t}^{+})^2 }{ n^{+}_t - 1}, \]
\[D^-_t = \frac{f^{2,-}_i(t) -2AVG_{i,t}^{-}f^{-}_i(t)  +n^{-}_t (AVG_{i,t}^{-})^2 }{ n^{-}_t - 1}.\]
By defining $\delta^+(t+1) =1$ if the $(t+1)$th instance is positive; otherwise $\delta^+(t+1) =0$, and $\delta^-(t+1)=1-\delta^+(t+1)$, the quantities of interest can be updated incrementally as follows:
\[ n^+_{t+1} = n^+_{t}+\delta^+(t+1) ,\ \ \  f^{+}_i(t+1) = f^{+}_i(t) + \delta^+(t+1) f^{j}_{i},\]
\[ f^{2,+}_i(t+1) = f^{2,+}_i(t) + (\delta^+(t+1) f^{j}_{i})^2.\]
\[ n^-_{t+1} = n^-_{t}+\delta^-(t+1) ,\ \ \  f^{-}_i(t+1) = f^{-}_i(t) + \delta^-(t+1) f^{j}_{i},\]
\[ f^{2,-}_i(t+1) = f^{2,-}_i(t) + (\delta^-(t+1) f^{j}_{i})^2.\]

It should be noticed that $n^+_t$ and $n^-_t$ do not depend on the feature index, while the other quantities do.



==> main.tex <==

\input{introduction.tex}

\input{fscore_inc.tex}

\input{background.tex}

\input{implementation.tex}

\input{experiments.tex}

\input{conclusions.tex}

\section{Acknowledgments}
This work was supported by the Italian Ministry of Education, University, and Research (MIUR) under \mbox{Project PRIN 2009 2009LNP494\_005.}

